Peekaboo: A Hub-Based Approach to Enable Transparency in Data Processing within Smart Homes (Extended Technical Report)

We present Peekaboo, a new privacy-sensitive architecture for smart homes that leverages an in-home hub to pre-process and minimize outgoing data in a structured and enforceable manner before sending it to external cloud servers. Peekaboo's key innovations are (1) abstracting common data pre-processing functionality into a small and fixed set of chainable operators, and (2) requiring that developers explicitly declare desired data collection behaviors (e.g., data granularity, destinations, conditions) in an application manifest, which also specifies how the operators are chained together. Given a manifest, Peekaboo assembles and executes a pre-processing pipeline using operators pre-loaded on the hub. In doing so, developers can collect smart home data on a need-to-know basis; third-party auditors can verify data collection behaviors; and the hub itself can offer a number of centralized privacy features to users across apps and devices, without additional effort from app developers. We present the design and implementation of Peekaboo, along with an evaluation of its coverage of smart home scenarios, system performance, data minimization, and example built-in privacy features.

==> Makefile <==
DOC = main-usenix.tex

OTHERSOURCES := $(filter-out $DOC, $(wildcard *.tex)) $(wildcard section/*.tex) \
  $(wildcard figure/*)

PDFLATEX = pdflatex -synctex=1 --shell-escape
BIBTEX = bibtex
RERUNBIB = "No file.*\.bbl|Citation.*undefined"
TARDIR = $(DOC:.tex=-src)

.PHONY: pdf clean

pdf: $(DOC:.tex=.pdf)

all: pdf

%.pdf: %.tex $(OTHERSOURCES)
	${PDFLATEX} $<
	egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(PDFLATEX) $<; $(PDFLATEX) $<) ; true

clean:
	@\rm -f \
        $(DOC:.tex=.aux) \
        $(DOC:.tex=.log) \
        $(DOC:.tex=.out) \
        $(DOC:.tex=.dvi) \
        $(DOC:.tex=.pdf) \
        $(DOC:.tex=.ps)  \
        $(DOC:.tex=.bbl) \
        $(DOC:.tex=.blg) \
        $(DOC:.tex=.synctex.gz) \
	$(DOC:.tex=-src.tar.gz)

veryclean: clean
	@\rm -r -f *~ *.log *.pdf *.gnuplot *.fdb_latexmk *.fls *.upa *.upb auto *.gz svg-inkscape

tar: pdf
	@test -d $(TARDIR) || mkdir $(TARDIR)
	@cp Makefile *.{tex,bib,bst,cls} $(TARDIR)
	@tar cz $(TARDIR) > $(TARDIR).tar.gz
	@rm -rf $(TARDIR)


==> parts/p5-privacy.tex <==
\section{Providing Independent Privacy Features through Architectural Support}\label{sec:privacyfeatures}

\name's architecture makes it possible for the hub to offer many kinds of privacy features by the hub itself, without any support from developers. We demonstrate three classes of privacy mechanisms below. 

Note that the privacy features described below are mainly to demonstrate the individual mechanisms. Some of them may potentially break a few apps' original functionality. Future developers can build more sophisticated features by combining some of the mechanisms. 


\subsection{Static analysis of the hub program}\label{sec:programsemanticanalysis}

A key advantage of using reusable operators as the common  structure is that these operators have well known semantics, making it easier to analyze/index the app behavior. 
We present two native privacy features that \name can offer through static analysis of hub programs.

The first one is \textit{Content-based permission management}, which is inspired by the privacy control mechanisms around permissions in smartphone OSs~\cite{felt2012android}. Android shows a user the list of permissions (e.g. access to the camera or microphone) requested by an app at install time, which a user needs to allow or deny. iOS provides modal dialogs when sensitive data is accessed rather than at install time. Both platforms allows these settings to be changed as well. 
However, applying the same paradigm of notifying users on the first access to sensitive data in the smart home system is less than ideal. First, in the case of smarthomes the apps often need continuous access to sensor data (e.g., the \textit{HelloVisitor} app) for their functionality and not just when an app is launched. Second, any form of binary controls to enable or disable access requires users to make a decision between functionality vs privacy, which in the smartphone ecosystem has been shown be as ineffective. Most importantly, the mobile permission system does not let the user to control the granularity of data shared with different apps (notable exception is fine grained vs coarse location) or controlling what data ultimately leaves their devices.



\begin{figure}
	\centering
	\includegraphics[width=\columnwidth]{figures/native-features.png}
	\caption{Peekaboo’s architecture makes it possible for the hub to offer many kinds of privacy features by the hub itself,without any support from developers. For example, the information inferred from the hub program's static analysis can support users' app download decision making. Indexing the apps by the type of outgoing content allows users to control the permissions through the setting menu. Finally, intercepting the runtime can quantify the actual outgoing data.}
	\label{fig:nativefeatures}
	\vspace*{-0.1in}
\end{figure}

\name's architecture makes it easy to offer a new type of permission management based on the outgoing content types. We formulate the content outgoing content permission as [content type] + [data type], such as \textit{raw image}, \textit{speech audio}. 
For example, the content egress permission for \textit{HelloVisitor} would be \textit{face image}. Users can interact with the content egress permission similarly to the mobile permissions, such as viewing the permissions at the installation time and controlling the permission through the setting menus (Fig.~\ref{fig:nativefeatures}). 

\name then uses a simple type system to automatically infer the required content egress permissions for each hub program.
Since each operator has clearly defined semantics, we can use the types of input data and the operator properties to infer the types of the output data. 
For example, the output data type of the \textit{retrieve pose} operator (Fig.~\ref{fig:retrieveoperator}) would be the \textit{pose tabular}, since the target content is \textit{pose} and the data type for the input pose data is \textit{tabular}.
We derive a set of type inference rules for each operator (see Table.~\ref{tab:operatorscategories}), and use these rules to annotate the types for each edge in the hub program. The required content egress permissions are the type annotations associated with network operators' output edges. Algorithm~\ref{alg:alg1} describes the process of the type annotations. 


\begin{algorithm}[!h]
	\caption{A type inference algorithm to deduce the content type flowing between operators progressively}	\label{alg:alg1}
	\begin{algorithmic}
	    \STATE \textbf{Goal}: To annotate the content/data types of the edges in a hub program progressively.. 
		\STATE \textbf{Input}: Let $G = (V, E)$ be a DAG representation of a hub program, where $V = [v_1, v_2, ...]$ is the set of vertices (i.e., operators), and $E = [e_1, e_2, ...] $ is the set of directed edges between vertices. 
		\STATE \textbf{Output}: The data flow inside each edge is an array of \name data items, and each data item is associated with a content type and a data type. We formulate the type annotation of each edge $e_i$ as $\psi_i = [(c_1, d_1), (c_2, d_2), ...]$, where $c_i$ and $d_i$ are the content type and data type, respectively. This algorithm wants to compute all the $\psi_i$.
		\STATE \textbf{Define}: $f(\phi, \psi) = \psi '$  is the type inference rule that maps the type annotations of the outgoing edge $\psi '$.  $ \phi $ is the operator's properties, and $ \psi $ is the type annotations of the incoming edge.
		\STATE \textbf{Begin} \\ %
		$V' \gets $ a topological ordering~\cite{10.1145/368996.369025} of $V$
		\FOR {each $v'$ in $V'$}
		 	\FOR {each edge $e_i$ in $v'$'s outgoing edges} 
		 			\IF {$v'$ has an incoming edge $e_j$} 
		 				\STATE $\psi' \gets \psi_j$
		 			\ELSE
		 				\STATE $\psi' \gets $ []
		 			\ENDIF 
		 			\STATE $\psi_i \gets f (\phi_i,  \psi')$
			\ENDFOR
		\ENDFOR
		\RETURN $[\psi_1, \psi_2, \psi_3, ...]$. 
	\end{algorithmic}
\end{algorithm}

Another example privacy feature we have built is an generator to generate privacy descriptions automatically based on the hub program, which can support users' decision making in installing a new \name app  (Fig.~\ref{fig:nativefeatures}). 
The generator produces an individual description for each network operator, and uses a simple and expressive template to explain when and what data is being sent to the cloud: 
\begin{equation} \{The \, app \,  sends \,  [\underline{content \,   permission} ] \, to \, \underline{[server]} \,  when \,  the \,  [\underline{Device}] \,  detect(s)  \,  [\underline{Target  \, content}] \, and | or \, ... \}
\end{equation} 
For example, the privacy description for the \textit{HelloVisitor} app is ``This app sends \underline{face images} to \underline{HelloVisitor.com} when \underline{the camera} detects \underline{a face}''. 
The generator first uses the network operator's property to fill the first half of the template, and then traverses the preceding operators to generate the conditional summary (i.e., when ...). 



During the traversing, if the generator finds any \textit{select} and \textit{retrieve} operators, the generator can use the operator's [\underline{target content}] to fill the template. \textit{select} and \textit{retrieve} are the only two operators that can change the program flow based on the content, so their [\underline{target content}] properties are the only properties that are relevant to the conditional summary . If there are multiple \textit{select}, \textit{retrieve}, and \textit{join - blocking}, the generator will continue to append $and$ to the description. If the generator finds a \textit{join - non-blocking}, the generator will append an $or$ to the end of the description. 


We can easily extend this template to more complex hub programs. For example, the privacy description of the baby crying monitoring app (Fig.~\ref{fig:appbabycrying}) would be as follows.

\textit{This app sends raw audio to www.abc.com when the microphone detects a baby crying sound.}




% \jason{Strongly suggest including a scenario with tabular data and another (simpler, not as complex as fall detection) scenario that goes beyond video. There were other scenarios mentioned in the intro but the paper never follows up on those.}
% To generate such a description, the generator first searches for the network operator and uses its property and the associated $[\underline{content \, permission} ]$  to fill the first half of the sentence. The generator generates individual descriptions for each network operator.  

% , where the \underline{face images} can be derived from the type system described above, the \underline{HelloVisitor.com} is documented in the \textit{send2cloud} operator. The context summary (i.e., when ...) can be computed by search for from the conditional filtering operators.  (\textit{select} and \textit{retrieve}) and the join operator. 



% \jason{This subsection lacks technical depth. Suggest sketching out how it works, and why it has a given format, e.g. 'does xxx when yyy'. More broadly, make sure that each of these sections is not just a description of what Peekaboo does, but also why (why it's useful plus design rationale). Need to convince readers that Peekaboo doesn't just offer privacy features, it offers useful privacy features.}

\subsection{Controlling the data behavior through program rewriting }\label{sec:programrewriting}

In \name, users have full control of their hub, and the data processing on the hub is structured through operators. These two properties makes it possible for the hub runtime to rewrite the hub program for users' privacy needs. 

The first feature is \textit{pull rate limiting}, which allows users to control the frequency at which a smart home app pulls data by modifying the operator properties.
For example, Figure~\ref{fig:waterleakfloor} illustrates the hub program of water leak detection app, which pulls an image from an existing smart camera every 30 minutes and sends only parts of the image with a floor in it to the server. Through the \textit{pull rate limiting}, the runtime can modify the property of the \textit{inject} operator from \textit{30 minutes} to \textit{120 minutes}, so the app only pull images every two hours. 


The second feature is \textit{discriminative face sharing}, which allows users to handle face data discriminatively by inserting operators to the hub program. Figure~\ref{fig:hubprogramextension} presents a modification to the HelloVisitor, which inserts a few operators between the \textit{crop face} operator and the \textit{send2cloud} operator. Instead of sending all the face images to the cloud, the modified program will only upload non-family members’ faces. The inserted subgraph can be appended to the \textit{crop face} operators in other hub programs as well. 


In contrast to the two features described in \S\ref{sec:programsemanticanalysis}, privacy features built through program rewriting are more powerful since they can directly control the behavior of the hub program, but are also less generalizable. For example, the \textit{pull rate limiting} can only apply to the apps triggered by an \textit{inject} timer, the \textit{discriminative face sharing} can only be applied to the hub program containing \textit{crop face} operators. 
Another caveat is that the misuse of these features on a wrong app may break the app's original functionality. 
One possible approach to leverage this capability is mapping specific features as the extensions to individual apps rather than a feature that can be enabled for any apps, since users may not have the expertise to debug the problem. 

% \jason{Generally, I can see that both of these are possible to do, but the paper needs to do much better in describing how to generalize these. The first scenario of rate limiting I could see since you only need to modify the initial operator. The second scenario you only need to modify the sendtocloud operator (or proxy the last one). I think that's the key here, that you can easily modify the chain of operators based on its initial input and final output to get additional privacy properties. If this is the key insight, then make that a lot more explicit. Don't just say 'we offer xyz', be like Yoda and offer wisdom and insight to your readers.}

\begin{figure}
	\centering
	\includegraphics[width=0.95\columnwidth]{figures/app-extended-hellovisitor-v2.eps}
	\caption{By inserting a subgraph of operators, \name can extend \textit{HelloVisitor} with a discriminative face sharing feature.}
	\label{fig:hubprogramextension}
	\vspace*{-0.1in}
\end{figure}




\subsection{Hub runtime interception}\label{sec:hubruntimeinterception}

% \jason{Similar comments as above for this section. Also, it feels to me that runtime interception and program rewriting are fairly similar. Data egress reports can be easily done by modifying the final sendtocloud operator or proxying it. Face spoofing seems harder though. Anyway, consider having only two categories of privacy features instead of three.}

Another important advantage of the \name architecture is that all the data processing is structured through operators and centralized in a hub, making it easier to intercept the actual data flowing between the operators as well as the outgoing data. 

The first feature using runtime interception is \textit{data egress reports}. Prior work on smartphones have shown the benefit of informing users about data egress such as privacy awareness, nudging them to manage privacy, and enhancing privacy controls \cite{almuhimedi2015your,van2017better,jin2018they}. However, implementing such features in conventional smart home architecture is increasingly difficult due to the inability to intercept encrypted traffic. Recent smart home privacy projects (e.g., IoT inspector~\cite{huang2020iot}) can only approximate the privacy egress through the number of network requests and the number of outgoing bytes. 


By intercepting the incoming data of each network operator, the hub runtime writes a log entry to a local database with a timestamp. By building a reverse index, the database can generate query responses like "In the past week, the HelloVisitor app had collected XX raw images for machine training, XX face images for person recognition." (Fig.~\ref{fig:nativefeatures})


Another example feature is \textit{face spoofing}, which is inspired by ProtectMyPrivacy~\cite{agarwal2013protectmyprivacy} which proposes giving anonymized data to smartphone apps. This feature intercepts the data flowing between operators and substitute the actual faces with fake ones, based on user preference. Imagine a user, who has numerous cameras used by multiple smart home apps, may want a global privacy policy that replaces all the outgoing images with faces with synthetic ones. In doing so, the hub runtime continually monitors the content in the memory and overwrites the data field in the memory if it finds a “face image” in the data flow.






% \jason{Going back to a comment above about a possible insight being just to modify the initial operator or final operator, I think you might be able to generalize this as a series of rules for transforming / modifying operator chains. Modifying initial and final is easy. Might also have a rule about faces too, e.g. if the chain has a face recognition operator, then insert a 'is it my face and if so spoof' operator between it and its output. This leads to a much more generalizable approach.}



% \jason{For Algorithm 1, it needs a much better name then 'annotating the context...'. Also, in the text above, try to convey the intuition of the algorithm rather than jumping to formalisms. What's the basic idea of how it works? Also, I don't get the output. Lastly, suggest adding something before 'input' which is 'goal'. What's the goal of the algorithm?}


%We develop two privacy features to demonstrate two types of program rewriting: property modification and operation insertion. 

%Water leak on the floor is a common problem in a residential place, and it may cause substantial damage if it is not handled quickly. The water leak detection app built using \name can leverage the existing security camera system and offered a water detection feature. However, streaming the full scene of the room to the server can expose undesired information, such as persons who appeared in the scene.

%Figure~\ref{fig:eval-app1} illustrates the hub program of water leak detection, which pulls an image from the associated camera every 30 minutes and sends only the floor segmentation to the server. 
%The app can lessen the impact of water leak problems by alerting the users when the events are detected, whether they are at home or away. 
%This app uses a pretrained MobileNetV2~\cite{zhou2018semantic} model for the floor segmentation and crops the image by setting the non-floor pixels black. We deployed and tested this app on a commercial Wyze camera~\cite{} with RTSP support.

%\name addresses this challenge by offering reusable network operators to aggregate encryptions tasks. In doing so, \name can defer the network data encryption after finishing the data analysis tasks. This design also offers benefits to developers since they no longer need to manage the encryption library patches themself. A recent study~\cite{huang2020iot} found that many device vendors often fall behind the TLS library patching schedules, exposing the communication to exploits from vulnerabilities. 


%\name indexes the five privacy properties of outgoing network requests through the network operators: which sensor provides the data, who (i.e., which app) is collecting data, what data, where that data is going, and why it is being collected. The sensor source (which) and app name (who) is documented in the metadata of the incoming data, and the server address (where) and purpose (why) are properties of the corresponding network operator. The data content (what) contains the actual inference results, e.g., the exact recognized speech text, which can be retrieved from the "inference" field in the incoming data. 



%\jason{Description here feels too basic. Could also use some more examples, to demonstrate the range of things that this supports.}

%\jason{Also, this feature feels really basic too, ie just logging. Is there any special insight here? Or rather that this architecture makes it much, much easier to do, and every app gets it for free, and that it's centralized so all of the data egresses from a single place and can be monitored.}


% \jason{For table below, suggest either cutting it or removing the first column of Feature 1 and Feature 2. The Feature 1 and 2 feels too weird to me. Also, if you keep it, add a caption.}
% \begin{tabular}{ ||  p{45mm}   | p{35mm}   | p{40mm}   || }
% 	\hline	\hline	
% 	 Program analysis (\S\ref{sec:programsemanticanalysis}) & Program rewriting (\S\ref{sec:programrewriting}) & Runtime interception (\S\ref{sec:hubruntimeinterception}) \\ \hline	
% Content egress permission &  Pull rate limiting & Face spoofing  \\ \hline	
%  Privacy description generation & Familiar face protection &  Data egress reports \\
% 	\hline	\hline	
% \end{tabular}
% \jason{Is there a better term than 'content egress permission'? Feels rather wordy and unclear as its meaning. } \YA{Maybe: Content Based Permissions to differentiate from the smartphone access permissions} 





% The type system annotates the [content type] and [data type] associated with each edge in the hub DAG. The required content egress permissions are the annotation of network operators' output. 

%\name uses a type system to automatically infer the necessary content egress permissions for each hub program. The input of the type system is the hub program manifest $ (V, E) $, and the output is a list of content egress permissions $C = [c_1, c_2, ...]$. 
%Given the content egress type of the incoming data and the operators' property, the type systems can infer the content egress type of the output data using a set of type inference rules (Table~\ref{tab:semanticrules1}). \name can only infer the content egress type of the output if the types of that operator' incoming data are known. So the type system starts with the root operators and analyzes the following operators' output progressively. 
%The required data egress types are the types associated with the network operators' output. Once the type system reaches a network operator, it appends the content egress permissions of the network operators' output to $C$. 


%it is difficult to extend this kind of mobile permission system to smart home scenarios, even if we assume all the apps run in an Android/iOS-like ecosystem. One important difference between the smartphone and smart home is that most smart home apps are sensor-driven, which require continuous access to those sensors (e.g., the \textit{HelloVisitor} app). Binary controls  (e.g., whether the HelloVisitor app can access the video doorbell) are insufficient since it either breaks the app functionality completely or requires users to give up their privacy. Besides, the mobile permission model only governs the data being accessed by the apps, but not necessarily the granularity of the data being sent out. Smart home apps may have legitimate needs to access the sensor, but it is not necessary to send all the retrieved data to external servers. 

%For example, when an Android user is installing a new app, the app store will show her a list of requested permissions to alert the mobile app's risks. Users can further toggle the app permissions to allow or deny data access. Android achieves this access control through a Dalvik virtual machine, which uses Linux group membership to govern device access rights. 

% Rewrote to make this clearer above. Leaving this in for clarity 
% However, it is difficult to extend this kind of mobile permission system to smart home scenarios, even if we assume all the apps run in an Android/iOS-like ecosystem. One important difference between the smartphone and smart home is that most smart home apps are sensor-driven, which require continuous access to those sensors (e.g., the \textit{HelloVisitor} app). Binary controls  (e.g., whether the HelloVisitor app can access the video doorbell) are insufficient since it either breaks the app functionality completely or requires users to give up their privacy. Besides, the mobile permission model only governs the data being accessed by the apps, but not necessarily the granularity of the data being sent out. Smart home apps may have legitimate needs to access the sensor, but it is not necessary to send all the retrieved data to external servers. 


%\begin{table*}[t!]
%	\renewcommand{\arraystretch}{1.2}
%	\begin{center}
%		\captionof{table}{The type inference rules to infer the content egress}   
%		\small 
%		\begin{tabular}{ || p{18mm} | p{30mm} | p{90mm} || }
%			\hline	\hline	
%			Data actions & Relevant properties & Behavior \\  \hline \hline
%			Pull \& Push & [datatype] & Append [raw] [datatype]  \\ \hline
%			Retrieve & [targetcontent] & Set  [DATA\_OVERVIEW] = [targetcontent], Clear other variables;  \\ \hline
%			Spoof \& Noisify& [targetcontent] & Append a new Filter statement F\_i; In F\_i, set [DATA\_CONTENT] = [targetcontent], [FILTERED] = "spoofed | noisify"; \\ \hline
%		    Select & [targetcontent] & Set  [DATA\_OVERVIEW] = [targetcontent]; Clear other variables; \\
%			\hline \hline
%		\end{tabular}
%		\label{tab:semanticrules1}
%	\end{center}
%\end{table*}

%\name makes the alerting mechanism feasible through two unique designs. First, the hub aggregates the common data preprocessing tasks across multiple apps, offering an ideal abstraction for privacy management. Second, \name introduces a new type of fine-grained permission for IoT privacy management, \textit{content permission}, which describes the granularity of the outgoing data content in natural languages, such as “an image where the faces are blurred,” “a speech text where the SSNs are spoofed.”
% \jason{May want to clarify that this is an extension of PrivacyStreams, since PrivacyStreams sort of does this. If so, should also clarify what the differences are. Also, want to clarify that this kind of permission is auto-generated based on the operators, right?}

% A typical content permission description contains two components. The first part describes the high-level categorization of the whole data object (e.g., a raw image, a voice audio, a speech text), and the second part contains a set of filtering statements (e.g., “all the face are blurred”), where the number of filtering statements can be 0 or multiple. \name formulates the description in the following data-to-text template: \begin{align}
% [DATA\_OVERVIEW] \hspace{0.3em} where \hspace{0.3em} [F_1, F_2, F_3, ..., F_i]
% \label{eq:1}
% \end{align}
% where
% \begin{align}
%  F_i (i.e., Filter \hspace{0.3em} statement) & = [DATA\_CONTENT] \hspace{0.3em} have \hspace{0.3em} been \hspace{0.3em} [FILTERED]\\
%  [DATA\_OVERVIEW] &= video \hspace{0.3em} | \hspace{0.3em} image \hspace{0.3em} | \hspace{0.3em} audio  \hspace{0.3em} | \hspace{0.3em} speech text  \hspace{0.3em} |  \hspace{0.3em} ...\\
%  [DATA\_CONTENT] &= face \hspace{0.3em} | \hspace{0.3em} SSNs  \hspace{0.3em} | \hspace{0.3em} ... \\
%  [FILTERED] &= blurred  \hspace{0.3em} |  \hspace{0.3em} spoofed  \hspace{0.3em} |  \hspace{0.3em} replaced  \hspace{0.3em} |  \hspace{0.3em} noisified  \hspace{0.3em} |  \hspace{0.3em} ...
% \end{align}

%\jason{I think it would be a stretch to call this program analysis. Maybe just say that its simple program analysis, which is doable bc of the known semantics of operators and fixed set of operators. Also, where are those filtered data\_content data\_overview metadata defined and stored? Also, what about more complex DAGs?}

%\jason{For this section, suggest giving a few examples of operator chains and showing what the outputs are. Id suggest maybe 5 plus examples, just so readers can get a better sense of things.}

%\name then leverages a type inference technique to infer these variables through static analysis automatically.
%At the core of the type inference is that each operator has a deterministic way in mapping the incoming data to the output data. For example, pull and pull operators (e.g., the getImage operator in Fig.~\ref{} ) always request the raw data, so the $DATA\_OVERVIEW$ of the output data is consistent with the corresponding “datatype” (e.g., image). A select operator (e.g., crop face)  maps the raw image input to the specified \textit{targetcontent} (i.e., a face image).  Table~\cite{} enumerates all the type inference rules. Given a hub program, \name first uses a breadth-first traversing algorithm to collect all root-to-leaf paths, and then applies the type inference rules to the operators in the paths sequentially. At the end, \name obtains a list of content permission variables for each network operator. Filling these variables into the template produces the list of content permission descriptions. 


% Traditionally, such an alerting mechanism can not apply to the IoT scenario for two reasons. First, there lacks a unified abstraction to manage the permission access, since the IoT devices are heterogeneous, distributed, and dynamic~\cite{schilit1995system}. 
% Second, many IoT apps require continuous data streams from few sensors~\cite{iotmud2062:online}. The device-based permission model (e.g., whether the HelloVisitor app can access the video doorbell) can only enable \textit{all or nothing} options, offering little value to privacy management.
%  \jason{Overall, this paragraph feels long and not super useful. Given space issues, suggest just getting to the main points more quickly.}

% The introduction of the reusable operators not only makes it easier for developers to implement data preprocessing tasks; more importantly, they also become the common structure of all the smart home apps. Privacy features built on these operators can apply to various apps, even if developers do not write any extra code. Further, these reusable operators come with known semantics, making it easier to analyze the app behavior. In this section, we demonstrate the feasibility of building native privacy features based on the common structure of operators. 

% Since the hub program is developed using a set of reusable operators with known semantics, and since all the data processing actions are centralized in a connected graph, it is easier to analyze the privacy-relevant behavior when compared to conventional cloud-based apps. 
% Through program analysis, \name enables two new privacy mechanisms: exposed data content inference and outgoing data report.
% \jason{Program analysis makes sense for the first item below, inference, but not for the second, which sounds like relatively standard logging.}

% and runtime enforcement through App Usage Description.

% Yet, enabling such a content-aware privacy mechanism is challenging.
% First, existing permission architectures often use a sandboxing mechanism (e.g., the Dalvik used by Android) to index the access to devices, but is incapable of offering content-level access control. Second, developers might not have a strong incentive to put effort into privacy enhancement, as improving it does not always provide direct benefits. For example, past developers find keeping the on-device machine learning model up-to-date hard~\cite{}.  

% In contrast, \name makes the privacy annotation (i.e., “who”, “where”, “what”, and “why”) of outgoing network requests a native feature.
% There still lacks a meaningful way to measure the data egress in the privacy content, since numbers of connections or the bytes of outgoing traffic can only approximate the privacy risks. 
% The second privacy feature we implemented in \name is the outgoing data report. The different with the exposed data content inference, \name places more emphasis on the actual data: what data has been actually sent to the developer. To do so, we aims to understand two features, what was contained in the raw images, how much information has been removed by the hub program, and what are the content has been sent to the program. 
% Every time the network nodes send a network request to the remote cloud, it will also write a log in the database. Combining that with the data content inference, we can build a reverse index, i.e., where can do what types of data has been sent to which developers, how much data has been request by a developer for a specific purpose. 

% As we can see, the content permission is characterized by the variables associated with the data egress (i.e., $DATA\_OVERVIEW, DATA\_CONTENT, FILTERED$). 
% for the hub program.   

% Given any hub program, \name generates the associated “exposed data content” property automatically using a combination of static analysis and data-to-text natural language generation template.

% As we described in \S\ref{}, each operator has a deterministic way to process the incoming data and generate the output data. By summarizing their behavior and semantic rule, we can infer the data granularity of the payload in each connection.

% Generating such a description involves the following basic steps:

% \haojian{I haven't got them done yet.}
% 
% \begin{itemize}[noitemsep,topsep=0pt]
% 	\item  Initialize two variables for the static analysis: [DATA\_TYPE] and an empty array which would be used to store the filter statement.
% 	\item  Recursively visit the following operators and update the variables using the semantic inference rules. 
% 	\item Fill the variables into the following data-to-text natural language generation template.
% \end{itemize}

% \name generates these descriptions by filling the result of static analysis into a data-to-text natural language generation template.


% \subsection{App usage description (MUD) enforcement}\label{sec:mud}
% => publish to MQTT (decide which apps can access). 
% => data sharing across the local apps; same developers; 
% => data sent to target service urls;
% => data sent for certain purposes; 








% As discussed earlier (\S\ref{}), completely isolating the data from developers to eliminate privacy concerns is not practical in many scenarios. Our position is aligned with recent privacy research (e.g., Privacy Expectation~\cite{}, Contextual Integrity~\cite{}), which found that “what people care most about is not simply restricting the flow of information but ensuring that it flows appropriately~\cite{}”. We aim to mitigate these concerns by developing a practical mechanism that can ensure the data flows appropriately.

% Note, the category is a categorization of the data sources with two critical implications. First, the four granularity is not necessarily associate with a privacy risk magnitude. Indeed, the derived information can be more privacy-sensitive than the partial raw category in some cases. Second, the categories are sensor dependent. For example, the lighting intensity can be the derived data for a camera sensor, but the raw data for the specialized lighting sensor.






%\subsection{End user interaction}
% transparency \& control

% All in One! User Perceptions on Centralized IoT Privacy Settings~\cite{marky2020all}


% A Data-Driven Approach to Designing for Privacy in Household IoT~\cite{he2019data}


% 1.  flow-based programming => automatically generate policy

%\subsection{Automatic privacy policy generation}
% Privacy compliance check 
% Run-time Permission is a must in *Android* Marshmallow. 
% The user will be happier allowing *permissions* because they are much more likely to install your app without a wall of *permissions* at the installation. The aim of this new model is to give the user full control over application's *permissions*.

==> parts/zp1-intro.tex <==
\section{Introduction}

For many smart home products, such as smart speakers, cameras, thermostats, and occupancy sensors, the ``brains'' of these systems are typically in the cloud. On-board sensors collect data and send them to remote servers, where key functionality (such as commands, analytics, or data sharing) typically happen. This cloud-based software architecture reduces the cost of IoT hardware, allows running computationally expensive algorithms, eases system/feature upgrades, and facilitates subscription-based business models. 

However, a major limitation of cloud-based IoT architectures is data privacy. Users have little control over the data transmission process, and in many cases, must either accept the fact that the proprietary hardware may collect raw data continuously, or simply not purchase these smart devices at all~\cite{Activate3:online, emami2019exploring}. 

Major smart home products are starting to offer increasingly comprehensive, also complex, privacy features. For example, the Alexa mobile app~\cite{Howtouse51:online} now allows users to manage their devices’ voice/alert/device history, and customize what information they want to share with various Alexa skills. However, building privacy support in these systems individually suffers from a few important limitations. 

\begin{itemize}[noitemsep,topsep=0pt]\label{list:limitations}
	\item Users can only manage their privacy through the functions implemented by the developers, which take a great deal of effort to build~\cite{}. Many smaller developers do not have resources to design and implement sophisticate privacy features~\cite{}.
	\item Third parties cannot verify if these privacy features work as claimed~\cite{}. 
	\item Different products might offer distributed and inconsistent sets of privacy features, imposing management challenges to users~\cite{dixon2012operating}.
\end{itemize}

This paper introduces \name, a new software architecture that can offer independent and verifiable privacy control and awareness. 
At the core of \name is two observations about smart home applications (\S\ref{sec:feasibility}). 
First, cloud services do not need raw data for many smart home scenarios. Indeed, developers often need to implement pre-processing functions (e.g., cropping face images, extracting audio frequency spectrum) repetitively on the cloud back-end to extract the desired data, so we can potentially factor out these pre-processing functions to a user-controlled hub.
Second, many pre-processing functions are common across applications, making it feasible to support them through a fixed set of reusable operators. 



\begin{figure*}
	\centering
	\includegraphics[width=2\columnwidth]{figures/computationshift-v3.eps}
	\caption{(a) In a conventional cloud-based architecture, the sensor sends the raw image to developers' servers, and developers need to implement a face detection algorithm to extract face images for further processing (e.g., face recognition, an online album with visitors' faces). (b) \name decouples the server program into two parts: a lightweight and elementary program running on the hub, and a custom and more computationally expensive program running on developers' servers. (c) The hub program can be implemented by connecting a fixed set of reusable operators into pipelines, where each operator is a “verb” statement corresponding to a data action (e.g., pull, detect, select, post). In doing so, \name reduces unnecessary data egress, offers a common structure to build unified and centralized privacy features, and alleviates the need to re-implement common data processing functionality.}
	\label{fig:sensorhubcloud}
	\vspace*{-0.1in}
\end{figure*}


In designing \name we propose three key ideas: hub, operators, and manifest.
First, \name helps developers factor out repetitive data pre-processing tasks from the cloud side onto a \textbf{user-controlled hub}, which will offer privacy features independently. 
Second, the pre-processing tasks on the hub can be implemented as a directed acyclic graph (DAG) of a fixed set of open-source, reusable, and chainable \textbf{operators}. 
Third, we represent the programs running on the hub (i.e., hub programs) as a text-based \textbf{manifest} file, which only stores the DAG' specifications, but not the actual implementation. Once a user installs a new manifest file, the \name hub compiles the actual executable code using preloaded operator implementations. 


Figure~\ref{fig:sensorhubcloud}a \& b illustrates two different implementations of a smart home app in the conventional cloud-based architecture and \name architecture. 
Imagine a video doorbell app named \textit{HelloVisitor}, which can recognize the person in front of a doorbell and track the visitor history. In a typical cloud-based implementation, the doorbell sends raw images to the cloud, and developers implement a preprocessing algorithm to extract face images for further processing. 
Although developers using conventional architecture can offer privacy protection in an aftereffect manner, this approach suffers from the four limitations briefed above. 

In contrast, the \name implementation (Figure~\ref{fig:sensorhubcloud}b) moves the face detection to the hub and implements it by wiring together four reusable operators (Figure~\ref{fig:sensorhubcloud}c). Once deployed, the camera streams the video to the hub, and the hub then pre-processes the video stream, only sending images with detected faces to cloud servers. 
Since these reusable operators have clearly defined semantics and since they are the common structure across apps, we can analyze and modify app behavior in ways that are not easily possible with conventional approaches, which typically involve arbitrary code.
In \S\ref{sec:privacyfeatures}, we present three mechanism primitives (program analysis, program rewriting, and runtime interception) to build privacy features based on these operators. 
For example, we can easily infer that the \textit{HelloVisitor} app needs to send \textit{face image} outside by analyzing the hub program (Fig.~\ref{fig:sensorhubcloud}c) statically. We can then insert an image blurring operator between the ``select face'' and ``post to cloud'', so the hub program will only send a blurred face image to the external server. \name can also inspect the runtime to count the actual number of face images sent by \textit{HelloVisitor}. 
These features can be generalized to all \name apps, without app developers having to write any extra code. 





%a new IoT app development framework to help developers build privacy-sensitive smart home apps. \name offers a hybrid architecture, where a local user-controlled hub pre-processes smart home data in a structured manner before relaying it to external cloud servers (Fig.~\ref{fig:sensorhubcloud}b). For example, imagine a video doorbell app named \textit{HelloVisitor}, which can recognize the person in front of a doorbell, customize the welcome voice message, and track the visitor history. Figure~\ref{fig:sensorhubcloud}a illustrates a typical cloud-based implementation, where the doorbell sends raw images to the cloud, and developers implement a face detection algorithm to extract face images for further processing. 

%In designing \name we propose three key ideas. 
%First, \name helps developers factor out repetitive data pre-processing tasks (e.g., face detection) from the cloud side onto a \textbf{user-controlled hub}. This design has a positive side effect of reducing unnecessary data egress, since the hub pre-processes the data before sending it to any cloud servers.
%Second, \name supports the implementation of these pre-processing tasks through a fixed set of open-source, reusable, and chainable \textbf{operators}. This design makes it easier to reason about the privacy-related behavior of an app (e.g., what data is being sent and when) because the semantics of these operators are well known. This approach also  alleviates the need for each app to re-implement common functionality.
%Third, we represent the programs running on the hub (i.e., hub programs) as a text-based \textbf{manifest} file, which only stores the operators' specifications, but not the operators' actual implementation. Once the runtime downloads a manifest file, it then fetches the public implementations of necessary operators. This manifest design allows the public to inspect the actual data behavior in a white box manner.


%In addition, users can only manage their privacy through the functions implemented by the developers, which take a great deal of effort to build, if the developers even considered privacy at all. Further, different product development teams might offer different sets of privacy features and different user interfaces, leading to a great deal of inconsistency~\cite{dixon2012operating}.



%This new software architecture presents us with new challenges to make it practical as well as opportunities to leverage its unique properties. 
%% First, can a small set of operators actually cover a wide variety of smart home use cases? Related, can these operators be feasibly run on a hub (as opposed to a powerful server)?
%We need to determine whether there is a finite set of common pre-processing tasks that can cover a wide variety of smart home use cases and whether we can move these tasks to the hub (\S\ref{sec:feasibility}). To understand whether this is feasible, 
%we first review the architectural constraints of a user-controlled hub and then analyze over 200 unique smart home use cases. Our results show that 85\% of these use cases can outsource pre-processing functions to the hub, and we can cluster these functions by the types of input and output data.


%Second, we need to design and enumerate the set of reusable operators and devise the grammar to assemble the operators into hub programs. The operators need to be implemented once and can then be reused, combined, and tailored for many applications. Combining these operators should allow developers to implement hub programs for most smart home use cases. Meanwhile, the operator should provide encapsulation of the most data pre-processing tasks, and the programmer does not need to know the inner workings of an operator to use it. Best practices in API design~\cite{bloch2006design} guide the design of our programming interfaces (\S\ref{sec:peekabooapi}): we started with a few use cases, then coded them using our initial API, and iterated on the API as we expanded the supported use cases. We finally concluded with 16 unique operators, where each operator is a ``verb'' statement corresponding to a data action. Figure~\ref{fig:sensorhubcloud}c demonstrates an example of using 4 of the operators (i.e., pull, detect, select, post) to implement a face extracting function on the hub. 

%Along with these challenges also comes an exciting opportunity. 

We implement a prototype of \name by leveraging a visual programming platform named Node-Red~\cite{NodeRED78:online}, and develop the operators as a set of Node-Red compatible building blocks. Developers can use the mature Node-Red web-based editor to build the hub program manifest file. In \S\ref{sec:implementation}, we introduce the end-to-end design of the \name runtime, describing how \name configures and executes the hub programs as operator manifests, routes the data through \name drivers, and reuses intermediate computation to optimize the computation resources.


We deploy the \name runtime using a Raspberry Pi connected to a TPU accelerator. 
We also present three case studies (\S\ref{sec:casestudies}) to demonstrate the end-to-end implementation of \name apps: smart TV usage logs, voice assistant, and home office productivity tracking. To understand the feasibility and benefits of the \name architecture, we then use these apps as a lens to evaluate the latency (\S\ref{sec:latency}), computation loads (\S\ref{sec:computationloads}), and privacy benefits (\S\ref{sec:privacybenefits}). We also conduct an online user study (\S\ref{sec:zoomstudy}) to test the usability of \name APIs with developers. Our results show that developers can indeed understand how to use \name quickly and complete programming tasks efficiently and correctly. 

This paper makes the following research contributions: 
\begin{itemize}[noitemsep,topsep=0pt]
	\item We introduce a new software architecture that factors out common data preprocessing functions from the cloud service side onto a user-controlled hub, supports these functions through a set of reusable, chainable, open-source operators, and represents the hub program as operator manifests. This architecture can potentially reduce unnecessary data egress, open the black box of smart home products' data behavior,  offer a common structure to build generalizable privacy features, and alleviates the need to re-implement common data processing functionality.
	\item We collect over 200 unique smart home use cases through a design fiction interview and literature review. We then analyze the feasibility of factoring their data preprocessing functions to the hub and supporting them using reusable operators. Our results show that most of these use cases share a set of common data preprocessing functions, which can potentially be moved to the hub. These findings demonstrate the need for, and informed the design of, \name.
	\item We introduce a taxonomy of reusable operators as the cornerstone of supporting the common data preprocessing functions, where each operator is a ``verb'' statement corresponding to a data action. We demonstrate the functionality and usability of the operators through both example demonstrations and user studies with developers, showing that \name can offer significant flexibility and reduce the amount of potentially sensitive data sent to cloud services. 
	\item We introduce three classes of privacy mechanisms (program analysis, program rewriting, and runtime interception) that can be directly offered by the hub itself because of our architecture. We demonstrate two example features for each of these classes.  
\end{itemize}


% Third, building a runtime to execute these operators is another daunting task. First, the developers build the hub program without knowing users’ actual hardware setup and have no direct access to the hub to configure the programs. Second, the hub has relatively limited computation resources, requiring \name to allocate the computing resources thriftily. In \S\ref{sec:runtime}, we introduce the end-to-end design of \name runtime, describing how \name configures and executes the hub programs as operator manifests, routes the data through \name drivers, and reuses intermediate computation to optimize the computation resources.
% \jason{Not clear what an operator manifest is at this point. Also, this point takes the focus away from privacy. Suggest just cutting it. Can still talk about it later on, but suggest not making it a focus in the intro.}


% \section{A running example of HelloVisitor in \name ecosystem}



% \jason{Lastly, readers don't get a sense as to the range of operators beyond what's in Fig 1. Suggest trying to convey these just a little.}
% , where the TPU is used to speed up all the deep learning inferences. 
% \jason{This point about TPU also relates to range of operators. This is the first mention of deep learning, and as a reader, I'm going, why are they bringing up deep learning here? The paper needs to make more of an explicit connection between the operators and deep learning.}

% \jason{These challenges are running really long. Suggest shortening them a lot. See if you can keep it to just one paragraph too. Also, better if the challenges are linked to the research contributions in a 1-1 mapping. }
% \haojian{I am currently uses a challenge structure. So each paragraph maps to a main section in the paper. }
% Second, we need to design and enumerate the fixed set of reusable operators. The operators need to be implemented once and can then be reused, combined, and tailored for many applications. Meanwhile, the operator should provide encapsulation of the most data pre-processing tasks, and the programmer does not need to know the inner workings of an operator to use it. 
% However, there are several key challenges that need to be addressed with our approach.

% \jason{Second item here needs to be phrased in the form of a challenge. I don't know what the problem to be solved is here.}
% Second, the idea of \name operators is similar in spirit to Unix pipes but differs in one essential design: the chained operators in a pipeline are structured processes with clearly defined data behavior \jason{how about 'semantics' instead?}, rather than the arbitrary implementation in Unix Pipes. 
% The operators need to be implemented once and can then be reused, combined, and tailored for many applications. Meanwhile, the operator should provide encapsulation of the most data pre-processing tasks, and the programmer does not need to know the inner workings of an operator to use it. 
% \jason{I'm not really understanding the argument above, it still all sounds like exactly Unix pipes.}

% Second, \name supports the implementation of these pre-processing tasks through a fixed set of reusable operators, which alleviates the need to re-implement common data pre-processing functionality. 
% Third, these reusable operators are common across all \name apps, and hence reasoning about their privacy features can be done without the app developers having to write any extra code. 
% \jason{I think better to say that the three key ideas are having a hub, operators to pre-process data in a structured way, and manifest. For the points above, can add them to point two about operators.}
% \jason{Try to convey at the end of this paragraph how these ideas lead to better privacy.}
% \jason{I think this point about most apps not needing access to raw data should be mentioned more in the intro. This is really the first mention of it in the paper, and it's a critically important point. Also, clarify that raw data means both sensor data as well as log data. The emphasis on Fig 1 may mislead readers into thinking that it's just camera data.}
% 	\haojian{The reason I downplay this argument is because I feel this argument applies to PrivacyStream but not the IoT Hub content. It's not the apps not needing access to raw data. The underlying fact is that we can move some of the preprocessing to the hub. I am considering to replace this argument completely.}

% \jason{I think the paper should really mention PrivacyStreams somewhere in the intro, and draw a contrast between that work and this one}
% \haojian{I can not figured out a good place to mention privacystream in the intro}.

% \jason{I think around here or next paragraph, can mention that these operators let us pre-processes data in a structured manner, offering x y and z (in constrast to arbitrary code)}

% \jason{Somewhere in the paper, maybe here or in the intro, might want to say that the operators are inspired by Unix pipes, but in some ways are more structured. Might also preview that we can translate things into natural language statements.}


% First, we need to confine the types of computations that can be moved to the hub and verify whether these computations can be implemented through reusable operators (\S\ref{sec:feasibility})
% \jason{I think this is not the right framing for operators, instead suggest saying that we need a flexible set that can cover the vast majority of use cases for IoT apps and devices}. Introducing a user-controlled hub between the devices and the cloud has several important implications, such as limited computation resources, lacking direct access to update the software, etc \jason{I don't understand the point you want to convey here about hub, it feels not needed for the smart home cases}. 

% Figure~\ref{fig:sensorhubcloud}a \& b illustrates two different implementations of an example smart video doorbell app, \textit{HelloVisitor}, which looks to recognize the person in front of the doorbell, potentially customize the welcome voice message, and track the visitor history. 

% We note that these features of the app only requires cropped faces rather than the entire raw image. In the cloud-based architecture (Figure~\ref{fig:sensorhubcloud} a), developers need to implement face detection on their server to extract the desired data. In contrast, 


% \jason{Maybe here can mention that it's a hybrid architecture, doing some things locally while also still allowing some things to be done remote. Might also answer the question above here, ie why still support cloud services?} \YA{I agree, and better to give some examples around the same Hello Visitor app that needs the cloud. could be to interface with other notification services, keep a log of the data, store the image, etc} 

%\textit{HelloVisitor} in \name and a conventional cloud-based architecture. \textit{HelloVisitor} is a video doorbell app that can recognize the person in front of the doorbell, customize the welcome voice message, and track the visitor history. 

% This paper introduces \name, a new IoT app development framework to help developers build privacy-sensitive smart home apps through the intermediary of a user-controlled hub\footnote{The hub can be any computing resource that serve as an intermediary between devices in the home and cloud services and is fully controlled by end-users, e.g., a Raspberry Pi, an old computer in the home, or a shared EC2 instance in the cloud.}.

% However, even if these frameworks are widely adopted, building privacy-sensitive smart home products remains challenging. 
% Imagine a smart camera that offers a federated learning option, which claims that it only uploads the weights rather than the images. Developers need to build from scratch the algorithm implementation on the edge and the cloud, as well as the accompanying management interface. Users then have to face distributed privacy control across different products and can hardly verify the actual data collection behavior since the proprietary hardware works as a black box.
% \jason{Suggest emphasizing this latter part more (end-user verification) and less of the former. Focus on the weak points of these existing solutions where Peekaboo does much better.}
% \jason{Need to clarify, why still support cloud services with Peekaboo? What's wrong with doing everything locally? }

% \jason{For Fig 1, be sure to create a more consistent visual language that will make it easier for folks to understand. I also still don't really like how Face extraction points to another box, I feel that makes it feel too indirect, but ok if you can't figure out another layout to make it work.}
% We also profile the system performance to show the feasibility of running the apps on a Raspberry Pi.
% \jason{This last sentence feels weak. Running apps on a Raspberry Pi doesn't sound challenging. Need to better describe what's interesting here / what the insight is.}
% The rest of this paper describes our solutions to the key challenges in making the above design practical. First, we propose a new app structure to orchestrate three distributed computing resources (edge devices, the hub, and cloud servers) and a manifest design to stitch operators into hub programs (\S\ref{sec:programpartition}). Second, we show how operators can be implemented once and reused, combined, and/or tailored for use in many applications (\S\ref{sec:peekabooapi}). Third, we demonstrate the feasibility of building a unified and centralized nexus for privacy awareness and control based on the common structure of operators (\S\ref{sec:privacyfeatures}).
% \jason{The flow of the paper breaks down here with this above paragraph. Typically, 'The rest of this paper' is the last paragraph of the intro. The paragraph below also feels out of place, can move this to an Implementation section.}


% In this paper, we introduce a new IoT app development framework named \name, which aims to make it easier to build privacy-sensitive smart home apps through the intermediary of a smart home hub. There are three key ideas behind \name. First, \name allows developers to factor out repetitive data preprocessing tasks (e.g., face detection, frequency spectrum extraction) from the cloud side onto a user-controlled hub. Second, \name supports the implementation of these preprocessing tasks through a fixed set of reusable operators. Third, these reusable operators become the common structure of all the \name apps, so privacy features built based on the operators can be reusable across all the Peekaboo apps, and app developers do not need to write any extra code. Meanwhile, each operator has clearly defined semantics, making it possible to build privacy features by analyzing, intercepting, and rewriting the app behavior. 

% \jason{For Fig 1, consider developing a visual language to differentiate between sensors, apps, data, and operators. Everything is the same-sized rectangle, making it hard to differentiate things. }

% \name's software architecture offers several benefits. 
% (1) \name can lower the barrier for privacy-sensitive smart home app development, since developers can utilize these system-wide reusable operators, alleviating the need to re-implement common data preprocessing functionality \jason{Suggest moving this to last, since the focus of paper will be on privacy}. (2) \name makes it easier for developers to get the data at the granularity they actually need for their app (e.g., face images for \textit{HelloVisitor} (Fig.~\ref{fig:sensorhubcloud})), rather than raw data. This feature also has a positive side effect of reducing unnecessary data egress
% \jason{I think this point may be hard for readers to get at this point in the paper. I think you may want to go thru a short example first and then come back to benefits.}
% (3) Each operator is open source and has a deterministic \jason{Suggest change 'deterministic' to 'clearly defined semantics'}
% \jason{Also, I think the essential part for oeprators is not that they are open source, but rather they are trusted, with open source being one way of achieving trust.} semantic, making it possible to automatically analyze the app behavior. \jason{I suspect this last point might be hard for readers to get as is, so may want to convey how this works with Fig 1}
% (4) Since these operators become the common structure across IoT apps, privacy features built based on the \name operators can be reusable across all the \name apps, and app developers do not need to write any extra code.
% \jason{Similar comment as above here for this point too}

% \jason{For Fig 1, if the main emphasis of the paper is on privacy, then suggest highlighting the key privacy features you get. Can use a different font / color to help highlight these.}

% Through analyzing over 200 unique smart home use cases, we found that most IoT scenarios do not need raw sensor data (see \S\ref{sec:understandingdatarequirement}). For example, to implement the person recognition and online visitor album features in a video doorbell app named \textit{HelloVisitor} (Fig.~\ref{fig:sensorhubcloud}), developers only need face images rather than the raw images, which might incidentally include packages on the floor, a home address, parked vehicles, and passersby. Similarly, to implement an \textit{occupancy detection} app on a microphone, developers only need frequency spectrum rather than raw audio, which might unintentionally include user conversations and sensitive activity sounds. 

% In this paper, we introduce a new IoT app development framework named \name, which aims to make it easier to build privacy-sensitive smart home apps through the intermediary of a user-controlled hub. 
% \jason{Suggest around here, say that there are NNN key ideas to Peekaboo. My take would be: (1) a trusted smart home hub, (2) operators for pre-processing data before it leaves, (3) manifest for apps that specify a chain of operators for each possible flow of outgoing data (similar to having an explicitly defined API for an IoT app or device). Then, can proceed with the rest of the text below, describing things in more detail}
%  \name's architectural design philosophy is to factor out repetitive data preprocessing tasks (e.g., face detection, frequency spectrum extraction) from the cloud side onto a user-controlled hub, and support them as a fixed set of open source, reusable, and chainable operators. These operators preprocess raw data to remove unneeded sensitive user information before the data flow to the cloud (and out of the users' control), thus reducing data egress and many potential privacy risks for users.

% which aims to make it much easier for developers to get the granularity of data they actually need rather than always requesting raw data, while simultaneously offering architectural support for privacy features across all the apps


% \textbf{Implementation}. 

% \textbf{Evaluation}. We evaluate \name from three perspectives. (1)  We implemented 3 smart home applications (water leak detection, smart voice assitant, and home office productivity tracking) using \name API, to demonstrate the expressiveness of \name API by creating multiple variations for each.
% (2) For each application, we use public data sets to evaluate the data egress reduction quantitatively. We demonstrated that \name applications can protect users from undesired speaker recognition, speech recognition and face detection in XX\%, XX\%, XX\%, XX\% of outgoing data requests, respectively. 
% (3) We implemented three system-level privacy features based on the \name operators, showing how \name can offer reusable privacy feature  to all smart home apps.


% evaluated \name over 3 different smart home apps built with \name

%: content-based permission control, privacy description auto-generation, and outgoing data report 

%explore the operators' design space and design a set of built-in operators that supports both implementation reuse and computation reuse . 

%The remainder of this paper is organized as follows. The system design of MobiPurpose is discussed in §2-4. We
%present our experiment and evaluation in §5-7, followed by a discussion of the related work in §8. We conclude
%with the limitations and design decisions of our system in §9-11.



% We develop a few system-level privacy features to demonstrate privacy reuse. \textit{Content permission} allows users to grant or revoke an apps' permission to the sensor data at the content level. For example, a user can control whether the app will have access to the face part in the video stream from a camera. 
% \textit{Privacy description auto-generation} can generate a short description to describe the data being collected and the collection context, such as "the app requests face images when someone appears in front of the camera", aiming to help users better understand the data behavior of the app. 
% \textit{Outgoing data report} can offer a data report for end-users, including information like "In the past week, the "HelloVisitor" app had collected XX raw images for machine training, XX face images for person recognition." 

% \swarun{A bit redundant.. sentences can be crisper. Also, I am missing some insights on why these are challenging per se from a research perspective. }


% \swarun{Except first bullet, rest are about evaluation. I'd like a concise description of whether anything other than the architecture itself (which is basically: pre-process data at the edge) is a research contribution. For example, design of the operators or user-facing privacy features}
% the contribution is the architecture + the development framework.

% \jason{Suggest two paragraphs here, one on implementation, and one on evaluation. To make things easier to skim, just use bullets for Contributions and not for the other parts (since we want to draw attention to contributions, but too many bullets makes that harder). Also, add some short boilerplate text for Contributions, e.g. ''}

% \jason{Also, in implementation, may want to foreground the importance of the manifest, which glues lots of these different parts together.}

% \begin{itemize}[noitemsep,topsep=0pt]
% 	\item \textbf{Content permission inference}. Each hub program's basic unit is reusable operators with known semantics, making it possible to analyze the program and index an app's behavior. Through analyzing the hub program, we can inform users of the granularity of the outgoing data in natural language descriptions, such as "an image where the faces are blurred," "a speech text where the SSNs are spoofed."
% 	\item \textbf{Outgoing data report}. Moving the preliminary content analysis components to the hub allows \name to inform users what data content has been actually sent out. \name can offer an outgoing data report for end-users, including information like “In the past week, the "HelloVisitor" app had collected XX raw images for machine training, XX face images for person recognition.”
% \end{itemize}

% TODO \jason{For Fig 1, suggest clarifying where different parts of the architecture live. That is, what is in one's home, and what is in the cloud.}
%hub becomes the gateway of all the outgoing network traffic and all the IoT apps share a common structure of the chainable operators. This
% \swarun{I liked the earlier ''forced to choose between''}
%\jason{Now I think about it some more, wouldn't thermostats and occupancy sensors do things locally, and just send usage data along? That is, another use case I've heard Googlers talk about for Nest is offering stronger guarantees to end-users as to what data / how summarized / how often data is phoned home to the mothership. This is a case you might also want to support (and could probably do so rather easily). For example, could also have an aggregator operator plus a gated timer operator, which just allows data every N seconds. I think this could be a really powerful feature... thinking about it some more, it's not just that we want to control a stream of data and its granularity, but also offer guarantees of all data that will leave a device, including sensor data, logs, etc. I think this could add more depth to the paper.}
%\haojian{The current programming interface does support this feature. But I implemented it in a different way. I want to design the hub as a memory-less system. So the data is only cached at the driver. I will go through it in the implementation section.}


% 	\item We introduce three new smart home privacy management mechanisms, which offer fine-grained privacy awareness and control that operates on the content of each sensor data request.
% \jason{Given that we did something like this for PrivacyStreams, I think it will be hard to claim it as a novel contribution. Instead, could say that we demonstrate two such examples of better privacy features that can come with all apps.}


% \swarun{This sentence is important.. but is best moved as a header for the next paragraph so that para 1 talks purely about developers. Also, this point must be mentioned earlier in your summary of \name\ paragraph - you are not just benefiting developers... you are also helping users. }
% \swarun{Start with a ``what challenge you are solving'' or ``what novel service you are offering'' sentence.. Something like.. A second key advantage of \name's architecture is that it allows users to have a direct and trusted understanding of the flow (or lack thereof) of their private data to different companies offering IoT services. }
% Further, \name introduces three new privacy management mechanisms for smart homes. First, through static program analysis, \name can inform users what data can be sent out, at what granularity, and where it will be sent. Second, \name can generate a Manufacturer Usage Description (MUD) using the hub program, which can be used to enforce the app behavior by a MUD controller. Third, by inspecting the outgoing data, \name can show users what data content has been sent out. \swarun{This paragraph is about the last sentence of the previous paragraph.. can you add captions to each something like.. How \name\ benefits developers for the first one and how \name\ benefits users for the second one.. } 

% The rest of this paper describes our solutions to the key challenges in making the above design feasible.
% \name first factors out these common data preprocessing functions from the cloud service side onto a user-controlled hub, so \name can reduce the amount of potentially sensitive data going to cloud services by only sending the preprocessed data to the cloud (\S\ref{sec:systemdesign}).
% Second, \name supports these hub programs through a set of reusable, chainable, trustable operators, so developers can avoid implementing repetitive functions (\S\ref{sec:peekabooapi}).
%  Finally, all the operators come with known semantics, making it possible for \name to offer privacy features at the system level (\S\ref{sec:privacyfeatures}). 
% \jason{'rest of paper' phrasing should only be in the intro. It's odd to use that phrasing when it's p7 already.}
% at the user-controlled hub, while shipping out only essential user data needed for the app to function to the cloud (and out of the users' control). 
% make it much easier for developers to build privacy-sensitive smart home apps. \swarun{One connecting sentence is missing here -- e.g. \name's architectural design philosophy is to pre-process raw data to remove unneeded sensitive user information at the IoT hub, while shipping out only essential user data needed for the app to function to the cloud. } 
% \name factors out \swarun{You should say: A privacy-sensitive app developer can leverage \name\ to factor out private information in a manner that users can verify.. otherwise it seems this process is automatic and developers are not involved. Then say that \name\ provides a library of common repetitive data pre-processing tasks at the hub that developers can chain together to achieve desired privacy goals. All of this is done in a way that allows multiple developers to co-exist efficiently + allows users to verifiably see which of their private data is being sent to which developers. } the repetitive data preprocessing tasks (e.g., face detection, frequency spectrum extraction) from the cloud side onto a user-controlled hub\footnote{The hub can be any computing resource that can intermediate between devices in the home and cloud services, and is fully controlled by end-users, e.g., a Raspberry Pi, an old computer in the home, or a shared EC2 instance in the cloud. For this paper, we will assume that the hub is a Raspberry Pi.}, supports them as a fixed set of trusted, reusable, and chainable operators, and then runs them over the sensor data before they flow to cloud services (and out of the users’ control). 
% \jason{Again, I think you will have a much stronger story if you go beyond just sensor data, but cover all of the possible reasons a device might connect back to the mothership and send data.}
% \haojian{I consider the log data a part of the sensor data as well.}
% \jason{Ok, though I don't think reviewers will read it that way. May want to make that more explicit.}
% \haojian{I will revisit them and adjust the terms.}


%  \swarun{Make these bullets crisper if possible}
% \jason{Ok this is probably the strongest version of the intro to date, nice work Haojian}
% \haojian{Thanks for your help and feedbacks.}

%	\item \textbf{System requirements beyond privacy}. Privacy is rarely the “only value” in app development. We revisit our framework design and discuss how \name handles the non-privacy system requirements. 
%	\jason{This feels a bit vague. Need to be clearer as to what was evaluated.}
% \swarun{Would be nice if you call these -- ``\name\ is developer-friendly'' ``\name\ protects user privacy'' or something like that.. keeping with the theme of helping developers + helping users}
% \haojian{I did not go with this pitch because I am concerned that reviewers may expect a developer user study.}
% developers to build privacy-sensitive smart home apps.
% The design philosophy
% \begin{itemize}[noitemsep,topsep=0pt]
% 	\item \name can lower the barrier for smart home app development, since developers can utilize these system-wide reusable operators, alleviating the need to re-implement common functionality.
% 	\item \name reduces unnecessary data egress without preventing developers from implementing planned features. For example, "HelloVisitor" developers can request only the face images instead of the raw picture, which may capture other undesired information, e.g., the package on the floor, the home address, and a parked vehicle. 
% 	\item The basic unit of each hub program is reusable operators with known semantics, making it possible to analyze the program and infer an app's behavior. This property further enables two new privacy management mechanisms for smart homes. When a user installs an app, \name can inform users of the required data content (e.g., face images). After installation, \name can show users what data content different apps are collecting (e.g., face images have been sent to the HelloVisitor app for X times).
% 	\item The hub becomes the gateway of all the outgoing network traffic, offering a unified and centralized privacy awareness and control for all the smart home apps. 
% \end{itemize}

% 	\jason{Need to mention this earlier in the intro. Readers won't know what this is.}

%This paper presents \name, a new IoT app development framework that aims to make it much easier for developers to build smart home apps in a manner that offers a great deal of flexibility while also minimizing the amount of potentially sensitive data going to cloud services. 
%Our key insight is that cloud services do not need raw sensor data for many IoT scenarios.
%\jason{Suggest add 1-2 examples of not needing raw sensor data here}
%\jason{Suggest moving the sentence below to the end of the paragraph. That is, talk about (a) most apps don't need raw data, (b) can have a hub that preprocesses data. Also, given that you mention how it makes developers lives easier via bullets later on, can just skip that for now, to make text shorter and less repetitive.}
%Indeed, developers often need to implement repetitive functions on the cloud back-end to extract the desired data, costing unnecessary development effort, bandwidth, and computational resources. 




%
%\name comes with a set of common operators, along with an operator taxonomy \jason{What does it mean that it comes with a taxonomy?}. Each operator is an open-sourced package, associated with one type of data action in the taxonomy. Developers can also create new operators and publish them in a package registry. 
%\jason{I really think this is going to raise a lot of question marks from reviewers, about how we know we can trust these operators, and we don't want reviewers to feel this way after the intro. I'd strongly suggest not putting this level of detail here, and instead say that, for this version, it's a fixed set of trusted operators, and talk about new operators in the discussion. For example, NPM showed how badly things can go with package registries for the web, with one publisher taking his code out and breaking hundreds of web sites.}

% Imagine a smart camera that offers a federated learning option, which claims that it only uploads the weights rather than the images. Users need to face distributed privacy control across different products and can hardly verify the actual data collection behavior since the proprietary hardware works as a black box.
% \jason{For the second half of this paragraph, link back to x, y, and z (ie why are things hard for end-users and developers, and how these existing solutions are insufficient)}



% Further, the combination of a hub and chainable operators offers a nexus for unified and centralized privacy management for all of one's smart home apps. On the one hand, each hub program's basic unit is reusable operators with known semantics, making it possible to analyze/enforce the app behavior. On the other hand, aggregating the content-relevant preprocessing functions as the common structure across smart home apps allows \name to offer privacy features 

% aggregating the common content-relevant preprocessing functions on the hub allows

% as the common structure in implementing IoT apps.

%  Ultimately, this property 

% the combination of a hub and chainable operators offers a nexus for unified and centralized privacy management for all of one's smart home apps: privacy features built based on the \name operators can be reusable across all the \name apps, while app developers do not need to write any extra code.


%Here, the provider operator (i.e., retrieve image) specifies the data retrieval behavior (e.g., pull v.s. push, frequency, resolutions) and gets raw sensor data from \name runtime. The inference operator (i.e., detect face) analyzes the raw data and derives content annotations \jason{Hard to understand this, clarify what this means}. The filter operator (i.e., crop face) filters the sensor data based on the content annotation. The outgoing network \jason{Awkward phrasing here} (i.e., send2cloud) is the only operator that has outgoing network access, which sends the data to the remote cloud. 


%\jason{Another way of talking about the above is, we are factoring out common functionality from the cloud service side of things onto the hub, which offers consistency and also lowers the barriers for app devs since they don't have to implement lots of the same functionality over and over, and consistency of UI.}


%\begin{figure}
%	\centering
%	\includegraphics[width=0.75\columnwidth]{figures/peekaboo-app.eps}
%	\caption{An example \name application for the "HelloVisitor" app. }
%	\label{fig:peekabooapplicationexample}
%	\vspace*{-0.1in}
%\end{figure}


% Existing IoT privacy-enhancing technologies tend to make a binary choice between either the developers' or the users' needs. For example, user-first solutions achieve perfect privacy protection~\cite{} by isolating the sensor data from developers completely, such as computing everything locally~\cite{lane2015zoe, Ondevice98:online}, processing on encrypted data in the cloud~\cite{gilad2016cryptonets}, or processing data in a remote sandbox~\cite{lee2019occlumency}. These solutions impose an extra cost to developers, in terms of development flexibility, computation efficiency, future maintainability, and expertise requirement, resulting in a low adoption in today's IoT development. In contrast, the widely adopted solutions (e.g.,~\cite{bahirat2018data,dixon2012operating}), which are easy for developers to implement and manage, send raw data to remote servers for processing and offer users an opt-out option. However, users have to face an all-or-nothing choice, since most IoT applications cannot run correctly if the sensor data is blocked. Indeed, there exists a gap for an easy-to-use programming framework that can also protect users' privacy pragmatically.



%Privacy permission management in smartphones has evolved significantly, while today’s IoT still uses a primitive privacy management model: all-or-nothing. A decade ago, smartphone users had to allow all requested permissions~\cite{TheEvolu45:online,Androidv30:online}  to install an app. Now, smartphone operation systems (e.g., iOS, Android) are offering a fine-grained runtime permission control. For example, an Uber user can decide whether to grant the location access in a pop-up window, which explains the data collection purpose~\cite{Requesti97:online}. In contrast, while Internet of Things (IoT) sensors in smart homes are collecting more intimate data than smartphones, users have little way to control privacy access. Users are complaining that they can only unplug the smart speaker to stop the “constantly on microphone”~\cite{Activate3:online}.


%At the heart of our solution is a new flow-based programming model, which can help developers in developing IoT applications and help users index the privacy access of different data streams. 
%\jason{What about scenarios outside of video? The text of the paper seems overly focused on video, but what about things like smart toys, ovens, voice assistants, lights, thermostats, etc?}
%Figure~\ref{fig:architecture} illustrates the architecture of our programming model, where each IoT application contains two components: an edge applet and a cloud program. The applets will run on an edge node where the users have full control. Developers can quickly build an edge applet by assembling chainable computing units from a public library. 
%If a user installs multiple IoT applications containing multiple edge applets, the edge node then automatically aggregates the edge applets of installed IoT apps into a flow.
%When a user makes a change to her privacy setting, the edge will update the flow accordingly. For example, the edge would remove the face blurring computing unit from the flow if the user allows the face access for a camera.  





%\begin{figure}
%	\centering
%	\includegraphics[width=1\columnwidth]{figures/permission_request_example.png}
%	\caption{A data-centric privacy management system allows users to grant permissions to IoT applications selectively. For example, users can decide whether the app "HelloVisitor" can access the face data in a video stream. If denied, the "HelloVisitor" will only receive a video stream with blurred faces.}
%	\label{fig:architecture}
%	\vspace*{-0.1in}
%\end{figure}




%A great deal of research has investigated alternative privacy-sensitive software architectures. One example approach is "do everything local", which avoids data collection by processing data locally at the edge where the data is being gathered~\cite{yu2018pinto, xu2018deeptype,he2019streaming}. For example, Google Pixel phones can run speech recognition entirely offline~\cite{he2019streaming, Googles25:online}. However, on-device IoT processing suffers from many disadvantages, comparing to the cloud-based architecture, such as insufficient computing resources~\cite{}, difficulties in updating the edge software~\cite{lin2016iot,jeffoverair:online}, security vulnerability due to misconfiguration~\cite{}, and energy costs~\cite{deng2016optimal}. Another alternative architecture is "trusted cloud computing", which protects users' privacy by introducing data protection mechanisms in the cloud, such as sandboxing~\cite{lee2019occlumency}, encrypted machine learning~\cite{gilad2016cryptonets}, federated machine learning~\cite{konevcny2016federated}, and data capsules~\cite{wang2019data} to name a few. However, this paradigm often adds significant overhead in computation, networking, and development, making it less practical for many IoT applications. 


==> parts/zp1-intro2.tex <==
\section{Introduction}

For many smart home products, such as smart speakers, cameras, thermostats, and occupancy sensors, the ``brains'' of these systems are typically in the cloud.
A major limitation of the cloud-based software architecture  is data privacy~\cite{wang2019riverbed}, since it is challenging to provide privacy assurances \textit{after} a user's private data has left the IoT device in her home. 

Having recognized the problem, both product teams and researchers has invented many new data minimization technologies, such as preventing data leaks by doing everything on the local device (e.g., Nest Max Hub~\cite{FAQsonca75:online}), reducing data leaks by sending only denatured content (e.g., Pinto~\cite{yu2018pinto}, RTFace~\cite{wang2017scalable}), and inventing new mechanisms to leverage trusted cloud computing resources (e.g., sandboxing~\cite{lee2019occlumency}, encrypted machine learning~\cite{gilad2016cryptonets}, and federated learning techniques~\cite{konevcny2016federated}). 

Despite much progress in these individual techniques, it remains challenging for companies to \textit{legitimately avoid collecting unnecessary smart home data while re-assuring users that this is indeed the case}. We summarize four main challenges below.\\
(1) \textbf{Coarse and aggressive data collection}.  Since updating cloud programs is much easier than updating software on edge devices, developers in practice still tend to collect the raw data aggressively and tailor the data for actual purposes on the cloud afterward.  \\
(2) \textbf{Limited transparency and behavior enforcement}. Both the hardware firmware and the service providers’ backend cloud servers are proprietary and black-boxes for consumers and privacy advocates, making it hard to verify and enforce the actual data collection behavior~\cite{Teardown30:online}.\\
(3) \textbf{Either siloed or naive management for users}. To manage data collection, existing solutions tend to choose between either being generic and naive or specialized and siloed. Generic solutions, such as network quarantine~\cite{sivaraman2015network}, can manage privacy across devices, but offers limited management granularity, putting users in an all-or-nothing situation. In contrast, specialized solutions can perform fine-grained privacy control (e.g., face blurring, audio spectrum extraction, temperature resolution reduction), but suffer from usability and reachability issues when users have devices from different vendors~\cite{dixon2012operating,khandelwal2021prisec}. \\
(4) \textbf{\textit{"Live off" on individual developers' privacy support}}. Users can only manage their privacy through the functions implemented by the developers, which takes a great deal of effort to build~\cite{}. Many smaller product teams do not have the resources to design and implement sophisticated privacy features~\cite{}.



\begin{figure*}
	\centering
	\includegraphics[width=2\columnwidth]{figures/peekaboo_overview-v1.eps}
	\caption{The architecture of a \name app named “HelloVisitor”. The developer authors a manifest using four chainable operators (i.e., push, detect, select, and post) and specifies the purpose as "the app needs face images to recognize identity and enable an online album." Once deployed, the camera streams the video to the hub, and the hub then pre-processes the video stream, only sending images with detected faces to cloud servers. Because the semantics of each operator is known, it is easy to analyze the privacy-related behavior of apps (e.g. “this app only sends images of faces to HelloVisitor.com”) and modify those behaviors if desired.}
	\label{fig:sensorhubcloud}
	\vspace*{-0.1in}
\end{figure*}

In this paper, we propose \name, a new software architecture that can 
\textit{help developers collect fine-grained data incrementally, while also making the process transparent, enforceable, centrally manageable, and extensible.} 
\name has three parts. The first is an in-home smart home \textbf{hub} that mediates access between edge devices and the wider Internet. The second is a \textbf{fixed} set of reusable and chainable \textbf{operators} for pre-processing data on the hub in a stream-orientated fashion. The third is developer-specified \textbf{manifests} that declare data pre-processing pipelines by wiring these chainable operators, as well as the fine-grained data collection purpose for each outgoing data flow.

Developers can mitigate conventional cloud-based applications (i.e., apps) into \name with minimal changes: (1) identify the pre-processing tasks (e.g., face detection) for each fine-grained data collection purpose; (2) factor these tasks from the cloud onto a local hub by declaring them in a manifest (e.g., Fig.~\ref{fig:sensorhubcloud}a).
Once the hub installs/updates a app, the hub downloads the manifest file and compiles a pre-processing program by loading local operator implementations that came with the runtime. In doing so, the hub acts as a fine-grained privacy firewall to pre-process smart home data in a \textit{structured} and \textit{enforceable} manner before relaying it to external cloud servers (Fig.~\ref{fig:sensorhubcloud}b). 

\name allows developers to configure the data collection behavior in a \textit{fine-grained} and \textit{incremental} manner through the manifest. In the conventional cloud-based architecture, it is relatively hard to update the data collection behavior in distributed edge devices, so data collections are often coarsely associated with many purposes. For example, smart camera developers often request the raw images, since they may use the images for multiple purposes (e.g., face images for person recognition, doorstep images for package detection), although each individual purpose only needs a portion of the raw data. \name changes the paradigm in two ways. First, developers can incrementally update the data collection behavior of a \name app by updating the manifest. Second, the manifest requires developers to associate each outgoing data flow with fine-grained data collection purposes, making it possible to justify the minimum data requirement for each outgoing data request and selectively block some of the data requests without breaking the key functionality.

\name makes the data collection process transparent and enforceable by combining the manifest with a fixed set of operators. In contrast to Android permission manifest, which enumerates all the protected resources, \name manifest allows developers to declare a data pre-processing pipeline by wiring a set of pre-loaded chainable operators. So a \name app can only do what it declares in the manifest, and the actual data collection behavior becomes transparent to third parties.

Indeed, \name runs a simple protocol on the hub (represented as a fixed set of operators), akin to the narrow waist of the IP protocol in the TCP/IP networking stack, widening to collect data from various internal edge IoT devices and relay the data to many external cloud services. 
While existing solutions often require an arduous process to aggregate low-level individual hardware APIs~\cite{dixon2012operating} or the distributed privacy control settings~\cite{khandelwal2021prisec}, \name can easily manage the information flow in a centralized and fine-grained manner through interacting with the narrow waist protocol.


Last but foremost, the \name hub can offer many kinds of privacy features by itself independently. Since the fixed set of operators have clearly defined semantics and since they are the common structure across apps, we can analyze and modify the information flow in ways that are not easily possible with conventional approaches, which typically involve arbitrary code. For example, we have built a simple static analyzer that can take a graph of operators and transform them into a simple natural language statement explaining what granularity of data will be sent out and to what third parties (e.g. “this app will pull audio data from a microphone every 5 minutes, estimate the loudness, and send it to sleep.com for sleep quality tracking”). 

%\name can also automatically generate IoT privacy nutrition labels based on the manifests, which will let end-users see information about individual apps. 
%Besides, \name also let end-users see what data has been sent to which  cloud service (e.g. as weekly reports), add rate limits (e.g. at most once every 10 minutes), and prevent certain kinds of data types from ever leaving (e.g. specific faces or events). 

The key challenges in making \name practical center around the design of the manifest and the fixed set of the operators, which needs to be expressive and reusable across a wide variety of smart home use cases, easy-to-author for developers, easy-to-comprehend for auditors, beneficial for privacy protection, and friendly with various program analysis techniques. To achieve these goals, we first conduct an in-depth analysis of over 200 unique smart home use cases and then iterate the API by coding these use cases incrementally. We finally conclude with 16 unique operators, where each operator is a “verb” statement corresponding to a data action. Figure~\ref{fig:sensorhubcloud} demonstrates an example of using 4 of the operators (i.e., pull, detect, select, post) to implement a face extracting manifest on the hub. 


We then implement a \name manifest authoring tool by leveraging a visual programming platform named Node-Red~\cite{NodeRED78:online}, and develop the operators as a set of Node-Red compatible building blocks. Developers can use the mature Node-Red web-based editor to author a manifest. 
We also build the end-to-end \name runtime, which can compile the manifest into an actual program, routing sensor data from edge devices to external servers. 

We conducted detailed experiments to evaluate \name’s system feasibility, developer usability, and privacy benefits. Our experiments reveal that: (1) \name is feasible to run on a low-cost deployment setup (<\$100) with commercial sensors; (2) Developers can understand the \name API quickly and author a new manifest correctly under 10 minutes. (3) \name can significantly reduce the data egress through the fine-grained data collection. (4) We implement three independent privacy features (privacy explanation generation, IoT nutrition label generation, data collection rate-limiting) to demonstrate how \name can offer independent privacy features across devices.
%We deploy the \name runtime using a Raspberry Pi connected to a TPU accelerator. 

\vspace*{0.02in}\noindent\textbf{Contributions}:   This paper contributes the following: 

\begin{itemize}[noitemsep,topsep=0pt]
	\item We introduce \name, a novel software architecture that can offer architectural support for building privacy-sensitive smart home apps. \name can help developers collect smart home data in a fine-grained and incremental manner, while also making the process transparent, enforceable, centrally manageable, and extensible. This architectural privacy support is enabled by a new interlocking mechanism among Hub, Manifest, and a fixed set of operators.
	\item We collect over 200 unique smart home use cases and analyze the feasibility of factoring their data pre-processing functions to the hub and supporting them using reusable operators. Our results show that most of these use cases share a set of common data pre-processing functions, which can potentially be moved to the hub. These findings demonstrate the need for, and informed the design of, Peekaboo. 
	\item We introduce a taxonomy of reusable operators as the cornerstone of supporting the common data
	pre-processing functions, where each operator is a “verb” statement corresponding to a data action. We demonstrate the functionality and usability of the operators through both example demonstrations and user studies with developers, showing that Peekaboo can offer significant flexibility and reduce the amount of potentially sensitive data sent to cloud services.
\end{itemize}


%The rest of this paper describes our solutions to the key challenges in making the above design practical. First, 
%In \S\ref{sec:implementation}, we introduce the end-to-end design of the \name runtime, describing how \name configures and executes the hub programs as operator manifests, routes the data through \name drivers, and reuses intermediate computation to optimize the computation resources.


==> parts/zp1-intro3.tex <==
\section{Introduction}



For many smart home products, such as smart speakers, cameras, thermostats, and occupancy sensors, the ``brains'' of these systems are typically in the cloud.
A major limitation of the cloud-based software architecture  is data privacy~\cite{wang2019riverbed}, since it is challenging to provide privacy assurances \textit{after} a user's private data has left the IoT device in her home. 

Having recognized the problem, both product teams and researchers has invented many new data minimization technologies, such as preventing data leaks by doing everything on the local device (e.g., Nest Max Hub~\cite{FAQsonca75:online}), reducing data leaks by sending only denatured content (e.g., Pinto~\cite{yu2018pinto}, RTFace~\cite{wang2017scalable}), and inventing new mechanisms to leverage trusted cloud computing resources (e.g., sandboxing~\cite{lee2019occlumency}, encrypted machine learning~\cite{gilad2016cryptonets}, and federated learning techniques~\cite{konevcny2016federated}). 

Despite much progress in these individual techniques, it remains challenging for companies to \textit{legitimately avoid collecting unnecessary smart home data while re-assure users that this is indeed the case} for following reasons. 
(1) To maximize the development flexibility, developers in practice still tend to collect the raw data aggressively and tailor the data for actual purposes on the cloud afterward.
(2) Users must trust IoT developers to collect their data appropriately, since both the hardware firmware and the service providers’ backend cloud servers are proprietary and black-boxes to third parties. 
(3) Manufactures often offer distributed and inconsistent sets of privacy features, imposing management challenges to users~\cite{dixon2012operating,khandelwal2021prisec}. 
(4) Many smaller developers do not have resources to design and implement sophisticated privacy features~\cite{}.


\begin{figure*}
	\centering
	\includegraphics[width=2\columnwidth]{figures/peekaboo_overview-v1.eps}
	\caption{The architecture of a \name app named “HelloVisitor”. The developer authors a manifest using four chainable operators (i.e., push, detect, select, and post) and specifies the purpose as "the app needs face images to recognize identity and enable an online album." Once deployed, the camera streams the video to the hub, and the hub then pre-processes the video stream, only sending images with detected faces to cloud servers. Because the semantics of each operator is known, it is easy to analyze the privacy-related behavior of apps (e.g. “this app only sends images of faces to HelloVisitor.com”) and modify those behaviors if desired.}
	\label{fig:sensorhubcloud}
	\vspace*{-0.1in}
\end{figure*}

This paper introduces \name, a new software architecture that can enable a sandboxed smart home environment to govern outgoing data for the sake of privacy. \name can provide many types of architectural support to build privacy-sensitive smart home apps. First, \name allows developers to collect smart home data on a need-to-know basis without sacrificing development flexibility. Developers can request only the data they actually need through \name, and easily update the data collection behavior to accommodate new usages incrementally. Second, \name allows third parties to verify the app data collection behavior without breaking the proprietary nature of IoT products, while also enforcing the app behavior. This can help consumers to build trust for devices from less reputed and intrinsically more privacy-invasive products. Third, \name ecosystem can build many native privacy features across devices, enabling all the \name apps to get them for free. Imagine a small team develops a new IoT product but focuses their energies on the primary functionalities, \name can save them effort on building many common privacy features, which are supported natively through \name. 


At the core of \name is an in-home hub that can act as a fine-grained privacy firewall to pre-process smart home data before relaying it to external cloud servers. For each \name app, developers can specify the fine-grained data requirements in a manifest. Once the hub installs/updates an app, the hub downloads the manifest and pre-process the raw sensor data into the targeting granularity. 
The main challenge in designing \name is defining the semantics of the manifest to describe the fine-grained data requirements in a unified and extensible manner and a policy enforcement mechanism that can enforce and verify the execution with low overhead. 


At first glance, one might consider adapting the existing sandbox manifests (e.g., Android permission manifest~\cite{} and Manufacturer Usage Description~\cite{}) for the smart home environment. Specifically, one can enumerate the required fine-grained data access (e.g., \textit{"ACCESS\_COARSE\_LOCATION"}) and a whitelist of Internet domains an app might contact in a manifest, and the hub will control the access to the corresponding APIs. Unfortunately, this approach does not scale well for the complexity of managing fine-grained data granularity in a smart home. A smart home contains many more sensors (e.g., cameras/microphones in the entrance/kitchen) than a smartphone, and many sensors require more granularities (e.g., face-only images, background-only images, pet-only images) than location sensors. Combining with the combo access (e.g., an app can only access the raw image if the microphone detects a falling sound.), the required number of permissions would be unwieldy for developers to use, and the number of APIs would be onerous for the hub to offer. 


In contrast to the traditional declarative permission manifest, \name allows developers to program imperative data-pre-processing pipelines directly inside the manifest, which query the data from sensors, pre-process it and relay it to external cloud servers. While offering developers more degree of freedom can address the complexity issue, it also makes the manifest hard to verify and inspect, even if the pre-processing code is public.
After analyzing over 200 IoT app scenarios from the research literature and by conducting design fiction interviews, we found that most pre-processing functions share similar data-agnostic data actions (e.g., detect can be a common data action for face detection, falling sound detection, abnormal temperature data detection). This observation motivates us to confine the programming API to author the pipeline: developers can only program a data pre-processing pipeline by wiring 16 pre-loaded chainable operators (Fig.~\ref{fig:sensorhubcloud}). So a \name app can only do what it declares in the manifest, and the actual data collection behavior becomes transparent to third parties.



%\name has three parts. The first is an in-home smart home \textbf{hub} that mediates access between edge devices and the wider Internet. The second is a \textbf{fixed} set of reusable and chainable \textbf{operators} for pre-processing data on the hub in a stream-orientated fashion. The third is developer-specified \textbf{manifests} that declare data pre-processing pipelines by wiring these chainable operators, as well as the fine-grained data collection purpose for each outgoing data flow.

%Developers can mitigate conventional cloud-based applications (i.e., apps) into \name with minimal changes: (1) identify the pre-processing tasks (e.g., face detection) for each fine-grained data collection purpose; (2) factor these tasks from the cloud onto a local hub by declaring them in a manifest (e.g., Fig.~\ref{fig:sensorhubcloud}a).
%Once the hub installs/updates a app, the hub downloads the manifest file and compiles a pre-processing program by loading local operator implementations that came with the runtime. In doing so, the hub acts as a fine-grained privacy firewall to pre-process smart home data in a \textit{structured} and \textit{enforceable} manner before relaying it to external cloud servers (Fig.~\ref{fig:sensorhubcloud}b). 

%\name allows developers to configure the data collection behavior in a \textit{fine-grained} and \textit{incremental} manner through the manifest. In the conventional cloud-based architecture, it is relatively hard to update the data collection behavior in distributed edge devices, so data collections are often coarsely associated with many purposes. For example, smart camera developers often request the raw images, since they may use the images for multiple purposes (e.g., face images for person recognition, doorstep images for package detection), although each individual purpose only needs a portion of the raw data. \name changes the paradigm in two ways. First, developers can incrementally update the data collection behavior of a \name app by updating the manifest. Second, the manifest requires developers to associate each outgoing data flow with fine-grained data collection purposes, making it possible to justify the minimum data requirement for each outgoing data request and selectively block some of the data requests without breaking the key functionality.

%\name makes the data collection process transparent and enforceable by combining the manifest with a fixed set of operators. In contrast to Android permission manifest, which enumerates all the protected resources, \name manifest allows developers to declare a data pre-processing pipeline by wiring a set of pre-loaded chainable operators. So a \name app can only do what it declares in the manifest, and the actual data collection behavior becomes transparent to third parties.

Indeed, \name runs a simple protocol on the hub (represented as a fixed set of operators), akin to the narrow waist of the IP protocol in the TCP/IP networking stack, widening to collect data from various internal edge IoT devices and relay the data to many external cloud services. 
While existing solutions often require an arduous process to aggregate low-level individual hardware APIs~\cite{dixon2012operating} or the distributed privacy control settings~\cite{khandelwal2021prisec}, \name can easily manage the information flow in a centralized and fine-grained manner through interacting with the narrow waist protocol.


Last but foremost, the \name hub can offer many kinds of privacy features by itself independently. Since the fixed set of operators have clearly defined semantics and since they are the common structure across apps, we can analyze and modify the information flow in ways that are not easily possible with conventional approaches, which typically involve arbitrary code. For example, we have built a simple static analyzer that can take a graph of operators and transform them into a simple natural language statement explaining what granularity of data will be sent out and to what third parties (e.g. “this app will pull audio data from a microphone every 5 minutes, estimate the loudness, and send it to sleep.com for sleep quality tracking”). 

%\name can also automatically generate IoT privacy nutrition labels based on the manifests, which will let end-users see information about individual apps. 
%Besides, \name also let end-users see what data has been sent to which  cloud service (e.g. as weekly reports), add rate limits (e.g. at most once every 10 minutes), and prevent certain kinds of data types from ever leaving (e.g. specific faces or events). 

%The key challenges in making \name practical center around the design of the manifest and the fixed set of the operators, which needs to be expressive and reusable across a wide variety of smart home use cases, easy-to-author for developers, easy-to-comprehend for auditors, beneficial for privacy protection, and friendly with various program analysis techniques. To achieve these goals, we first conduct an in-depth analysis of over 200 unique smart home use cases and then iterate the API by coding these use cases incrementally. We finally conclude with 16 unique operators, where each operator is a “verb” statement corresponding to a data action. Figure~\ref{fig:sensorhubcloud} demonstrates an example of using 4 of the operators (i.e., pull, detect, select, post) to implement a face extracting manifest on the hub. 


We implement a \name manifest authoring tool by leveraging a visual programming platform named Node-Red~\cite{NodeRED78:online}, and develop the operators as a set of Node-Red compatible building blocks. Developers can use the mature Node-Red web-based editor to author a manifest. 
We also build the end-to-end \name runtime, which can compile the manifest into an actual program, routing sensor data from edge devices to external servers. 

We conducted detailed experiments to evaluate \name’s system feasibility, developer usability, and privacy benefits. Our experiments reveal that: (1) \name is feasible to run on a low-cost deployment setup (<\$100) with commercial sensors; (2) Developers can understand the \name API quickly and author a new manifest correctly under 10 minutes. (3) \name can significantly reduce the data egress through the fine-grained data collection. (4) We implement three independent privacy features (privacy explanation generation, IoT nutrition label generation, data collection rate-limiting) to demonstrate how \name can offer independent privacy features across devices.
%We deploy the \name runtime using a Raspberry Pi connected to a TPU accelerator. 

\vspace*{0.02in}\noindent\textbf{Contributions}:   This paper contributes the following: 

\begin{itemize}[noitemsep,topsep=0pt]
	\item We introduce \name, a novel software architecture that can offer architectural support for building privacy-sensitive smart home apps. \name can help developers collect smart home data in a fine-grained and incremental manner, while also making the process transparent, enforceable, centrally manageable, and extensible. This architectural privacy support is enabled by a new interlocking mechanism among Hub, Manifest, and a fixed set of operators.
	\item We collect over 200 unique smart home use cases and analyze the feasibility of factoring their data pre-processing functions to the hub and supporting them using reusable operators. Our results show that most of these use cases share a set of common data pre-processing functions, which can potentially be moved to the hub. These findings demonstrate the need for, and informed the design of, Peekaboo. 
	\item We introduce a taxonomy of reusable operators as the cornerstone of supporting the common data
	pre-processing functions, where each operator is a “verb” statement corresponding to a data action. We demonstrate the functionality and usability of the operators through both example demonstrations and user studies with developers, showing that Peekaboo can offer significant flexibility and reduce the amount of potentially sensitive data sent to cloud services.
\end{itemize}




